A Comprehensive Survey on 6G Networks:Applications, Core Services, Enabling Technologies, and Future Challenges

Cellular Internet of Things (IoT) is considered as de facto paradigm to improve the communication and computation systems. Cellular IoT connects massive number of physical and virtual objects to the Internet using cellular networks. The latest generation of cellular networks, e.g. fifth-generation (5G), use evolutionary and revolutionary technologies to notably improve the performance of wireless networks. However, given the envisioned new use-cases, e.g., holographic communication, and the ever-increasing deployment of massive smart-physical end-devices in IoT, the volume of network traffic has considerably raised, and therefore, the current generation of mobile networks cannot wholly meet the ever-increasing demands. Hence, it is envisioned that the next generation, sixth generation (6G) networks, need to play a critical role to alleviate such challenges in IoT by providing new communication services, network capacity, and ultra-low latency communications (uRLLC). In this paper, first, the need for 6G networks is discussed. Then, the potential 6G requirements and trends, as well as the latest research activities related to 6G are introduced e.g., Tactile Internet and Terahertz (THz). Furthermore, the key performance indicators, applications, new services, and the potential key enabling technologies for 6G networks are presented. Finally, several potential unresolved challenges for future 6G networks are presented.

==> Sections/Enaling_Technologies.tex <==
\section{6G Enabling Technologies}\label{EnablingTechnologies}
This section investigates the technologies arising as enablers of the 6G network use cases and related KPI, discussed in Sections \ref{New service classes for 6G} and \ref{The key 6G KPIs and use cases}. One must note that, some of these technologies have already been considered or discussed in the 5G networks (i.e., evolutionary technologies); however, they are not commercially available for the 5G networks due to technological limitations or market boundaries. Regarding this fact, one can categorize these technologies into two major groups, including evolutionary (e.g., sparse signal processing) and revolutionary technologies (e.g., \gls{thz} communications). The 6G breakthroughs can happen in different layers (e.g., PHY), network architecture, communication protocols, network intelligence, etc. This section is dedicated to the evolutionary technologies of 6G. 
\input{Sections/Evolutionary_technologies}
\input{Sections/Revolutionary_technologies}

==> acro.tex <==
%\twocolumn
\tablehead{\toprule \makebox[.1\textwidth][c]{\textbf{Acronym}} \quad\quad\quad\quad\quad\quad\quad\quad{\textbf{Definition}} \\ 
    \\ \midrule}
\renewcommand{\arraystretch}{0.3}
    \scriptsize
\tablelasttail {\bottomrule}
\begin{xtabular}{p{0.45\textwidth}} 
\vspace{4ex}%[4ex]
\Acro{3cls}[3CLS]{Control, Localization, and Sensing}\\
\Acro{3gpp}[3GPP]{3rd generation partnership project}\\
\Acro{3d}[3D]{3-Dimensional}\\
\Acro{ai}[AI]{artificial intelligence}\\
\Acro{ar}[AR]{augmented reality}\\
%\Acro{aqmp}[AQMP]{Advanced Message Queuing Protocol}\\
\Acro{aid}[AID]{Autonomous intelligent driving}\\
\Acro{au}[AU]{aerial user}\\
\Acro{aes}[AES]{Advanced Encryption Standard}\\
\Acro{amp}[AMP]{approximate message passing}\\
\Acro{ap}[APs]{access points}\\
%\Acro{ssn}[SSN]{self-sustainable networks}\\
\Acro{cad}[CAD]{cooperative automated driving}\\
\Acro{csi}[CSI]{channel state information}\\
\Acro{cran}[CRAN]{cloud radio access network}\\
\Acro{dl}[DL]{deep learning}\\
\Acro{d2d}[D2D]{Device-to-device}\\
\Acro{embb}[eMBB]{enhanced mobile broadband}\\
\Acro{ecc}[ECC]{Elliptic Curve Encryption}\\
\Acro{em}[EM]{emit electromagnetic}\\
\Acro{ei}[EI]{Edge Intelligence}\\
\Acro{e2e}[E2E]{end-to-end}\\
\Acro{etsi}[ETSI]{European Telecommunications Standards Institute}\\
\Acro{gps}[GPS]{global positioning system}\\
%\Acro{gcs}[GCS]{ground control station}\\
%\Acro{hetnet}[HetNet]{Heterogeneous networks}\\
\Acro{hmimos}[HMIMOS]{holographic MIMO surface}\\
\Acro{iot}[IoT]{Internet of things}\\
\Acro{iiot}[IIoT]{industrial \ac{iot}}\\
\Acro{itu}[ITU]{International Telecommunication Union}\\
%\Acro{imu}[IMU]{inertial measurement unit}\\
\Acro{ict}[ICT]{Information and Communication Technology}\\
\Acro{ids}[IDS]{intrusion detection system}\\
\Acro{ir}[IR]{infrared}\\
\Acro{kpi}[KPI]{key performance indicator}\\
\Acro{los}[LoS]{line-of-sight}\\
%\Acro{lidar}[Lidar]{Light Detection and Ranging}\\
\Acro{lorawan}[LoRaWAN]{Long Range Wide Area Network}\\
\Acro{lis}[LIS]{Large Intelligent Surfaces}\\
\Acro{mimo}[MIMO]{multiple-input and multiple-output }\\
\Acro{mtc}[MTC]{machine-type communication}\\
\Acro{mmtc}[mMTC]{massive \ac{mtc}}\\
\Acro{mmi}[MMI]{mind-machine interface}\\
\Acro{mmwave}[mmWave]{millimetre wave}\\
\Acro{ml}[ML]{machine learning}\\
\Acro{mec}[MEC]{mobile edge computing}\\
\Acro{nfv}[NFV]{network function virtualization}\\
\Acro{nmo}[NMO]{Network Management and Orchestration}\\
%\Acro{nr}[NR]{new radio}\\
\Acro{ntc}[NTC]{network traffic classification}\\
\Acro{nbiot}[NB-IoT]{Narrow band \ac{iot}}\\
\Acro{ntp}[NTP]{network traffic prediction}\\
\Acro{ntma}[NTMA]{network traffic monitoring and analysis}\\
\Acro{noma}[NOMA]{Non-orthogonal multiple access}\\
\Acro{ofdm}[OFDM]{Orthogonal frequency-division multiplexing}\\
\Acro{owc}[OWC]{optical wireless communication}\\
%\Acro{oam}[OAM]{orbital angular momentum}\\
\Acro{oma}[OMA]{orthogonal multiple access}\\
%\Acro{phy}[PHY]{physical layer}\\
\Acro{plmn}[PLMN]{public land mobile network}\\
\Acro{qos}[QoS]{quality of service}\\
\Acro{qoe}[QoE]{quality of experience}\\
\Acro{qc}[QC]{quantum computing}\\
\Acro{qoc}[QOC]{quantum optical communication}\\
\Acro{qkd}[QKD]{quantum key distribution}\\
\Acro{ris}[RIS]{reconfigurable intelligent surfaces}\\
\Acro{rl}[RL]{reinforcement learning}\\
\Acro{ra}[RA]{Random Access}\\
\Acro{rf}[RF]{radio frequency}\\
%\Acro{rrm}[RMM]{radio resource management}\\
\Acro{sdn}[SDN]{software defined networking}\\
%\Acro{son}[SON]{Self-organizing Networks}\\
%\Acro{smtc}[sMTC]{super-reliable \ac{mtc}}\\
\Acro{sr}[SR]{super resolution}\\
\Acro{swap}[SWAP]{size/weight and power}\\
\Acro{sal}[SAL]{single-anchor localization}\\
\Acro{svm}[SVM]{support vector machine}\\
\Acro{sic}[SIC]{successive interference cancellation}\\
\Acro{thz}[THz]{Terahertz}\\
\Acro{urllc}[URLLC]{ultra-reliable low-latency communications}\\
\Acro{uhsllc}[uHSLLC]{ultra-high speed-with-low-latency communication }\\
\Acro{umub}[uMUB]{ubiquitous mobile ultra-broadband}\\
\Acro{uhdd}[UHDD]{ultra-high data density}\\
\Acro{uav}[UAV]{unmanned aerial vehicle}\\
\Acro{ue}[UE]{User Equipment}\\
\Acro{uv}[UV]{ultraviolet}\\
\Acro{udhn}[UDHN]{ultra-dense heterogeneous networks}\\
\Acro{v2x}[V2X]{vehicle to everything}\\
\Acro{vr}[VR]{virtual reality}\\
\Acro{vmr}[VMR]{virtual meeting room}\\
\Acro{vlc}[VLC]{visible light communication}\\
\Acro{wipt}[WIPT]{wireless information and power transfer}\\
\Acro{wpt}[WPT]{wireless power transfer}\\
\Acro{xr}[XR]{extended reality}\\
\label{tab:Acronyms}
\end{xtabular}
\normalsize
%\onecolumn

==> acronyms.tex <==
\makeglossaries

\newlength\maxlength
\newlength\thislength

\newglossarystyle{mystyle}
{%
  \renewenvironment{theglossary}%
  {% start of glossary
   % Find maximum width of the first column:
    \setlength{\maxlength}{0pt}%
    \forglsentries[\currentglossary]{\thislabel}%
    {%
       \settowidth{\thislength}{\glsentryshort{\thislabel}}%
       \ifdim\thislength>\maxlength
         \setlength{\maxlength}{\thislength}%
       \fi
    }%
    % Now calculate the width of the second column:
    \settowidth{\thislength}{\hspace{1.5em} \hspace{1em}}%
    \setlength{\glsdescwidth}{\linewidth-\maxlength-\thislength-2\tabcolsep}%
    % Start the tabular environment
    \begin{tabular}{l@{\hspace{1.5em} \hspace{1em}}p{\glsdescwidth}}
    \toprule
    \multicolumn{1}{l}{\textbf{Acronym}} &
    \multicolumn{1}{@{}l}{\textbf{Definition}}\\%
    \midrule
  }%
  {% end of glossary
     \bottomrule
     \end{tabular}%
  }%
  % Header has been incorporated into \begin{theglossary}
  \renewcommand*{\glossaryheader}{}%
  % Don't do anything between letter groups
  \renewcommand*{\glsgroupheading}[1]{}%
  \renewcommand*{\glsgroupskip}{}%
  % Set display for each the acronym entry
  \renewcommand{\glossentry}[2]{%
    \glstarget{##1}{\glsentryshort{##1}}% short form
    &
    \glsentrylong{##1}% long form
    \\% end of row
  }%
  % No sub-entries, so \subglossentry doesn't need redefining
}
\newacronym{nfv}{NFV}{network function virtualization}
\newacronym{sdn}{SDN}{software defined networking}
\newacronym{mimo}{MIMO}{multiple-input and multiple-output }
\newacronym{embb}{eMBB}{enhanced mobile broadband}
\newacronym{urllc}{URLLC}{ultra-reliable low-latency communications}
\newacronym{mtc}{MTC}{machine-type communication}
\newacronym{ofdm}{OFDM}{Orthogonal frequency-division multiplexing}
\newacronym{mmtc}{mMTC}{massive \gls{mtc}}
\newacronym{uhsllc}{uHSLLC}{ultra-high speed-with-low-latency communication }
\newacronym{iot}{IoT}{Internet of things}
\newacronym{umub}{uMUB}{ubiquitous mobile ultra-broadband}
\newacronym{uhdd}{uHDD}{ultra-high data density}
\newacronym{iiot}{IIoT}{industrial \gls{iot}}
\newacronym{v2x}{V2X}{vehicle to everything}
\newacronym{xr}{XR}{extended reality}
\newacronym{mmi}{MMI}{mind-machine interface}
\newacronym{ioe}{IoE}{Internet of everything}
\newacronym{kpi}{KPI}{key performance indicator}
\newacronym{mmwave}{mmWave}{millimetre wave}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ml}{ML}{machine learning}
\newacronym{ar}{AR}{augmented reality}
\newacronym{nmo}{NMO}{Network Management and Orchestration}
\newacronym{vr}{VR}{virtual reality}
\newacronym{nr}{NR}{new radio}
\newacronym{itu}{ITU}{International Telecommunication Union}

\newacronym{aqmp}{AQMP}{Advanced Message Queuing Protocol}
\newacronym{aid}{AID}{Autonomous intelligent driving}
\newacronym{3cls}{3CLS}{Control, Localization, and Sensing}
\

\newacronym{qos}{QoS}{quality of service}
\newacronym{qoe}{QoE}{quality of experience}
\newacronym{hetnet}{HetNet}{Heterog}
\newacronym{smtc}{sMTC}{super-reliable \gls{mtc}}
\newacronym{gps}{GPS}{global positioning system}
\newacronym{uav}{UAV}{unmanned aerial vehicle}
\newacronym{imu}{IMU}{inertial measurement unit}
\newacronym{gcs}{GCS}{ground control station}
\newacronym{vmr}{VMR}{virtual meeting room}
\newacronym{sr}{SR}{super resolution}
\newacronym{au}{AU}{aerial user}
\newacronym{bs}{BS}{base station}
\newacronym{los}{LoS}{line-of-sight}
\newacronym{ecc}{ECC}{Elliptic Curve Encryption}
\newacronym{swap}{SWAP}{size/weight and power}
\newacronym{3gpp}{3GPP}{3rd generation partnership project}
\newacronym{dl}{DL}{deep learning}
\newacronym{aes}{AES}{Advanced Encryption Standard}
\newacronym{ue}{UE}{User Equipment}
\newacronym{sal}{SAL}{single-anchor localization}
\newacronym{ris}{RIS}{reconfigurable intelligent surfaces}
\newacronym{rl}{RL}{reinforcement learning}
\newacronym{lidar}{Lidar}{Light Detection and Ranging}

\newacronym{svm}{SVM}{support vector machine}
\newacronym{ict}{ICT}{Information and Communication Technology}
\newacronym{lorawan}{LoRaWAN}{Long Range Wide Area Network}
\newacronym{ntc}{NTC}{network traffic classification}
\newacronym{3d}{3D}{3-Dimensional}
\newacronym{nbiot}{NB-IoT}{Narrow band \gls{iot}}
\newacronym{ntp}{NTP}{network traffic prediction}
\newacronym{ids}{IDS}{intrusion detection system}
\newacronym{cad}{CAD}{cooperative automated driving}
\newacronym{ntma}{NTMA}{network traffic monitoring and analysis}
\newacronym{phy}{PHY}{physical layer}
\newacronym{ann}{ANN}{artificial neural network}
\newacronym{ra}{RA}{Random Access}
\newacronym{rf}{RF}{radio frequency}
\newacronym{owc}{OWC}{optical wireless communication}
\newacronym{ir}{IR}{infrared}
\newacronym{uv}{UV}{ultraviolet}
\newacronym{vlc}{VLC}{visible light communication}
\newacronym{em}{EM}{emit electromagnetic}
\newacronym{its}{ITS}{intelligent transportation system}
\newacronym{wipt}{WIPT}{wireless information and power transfer}
\newacronym{qc}{QC}{quantum computing}
\newacronym{qoc}{QOC}{quantum optical communication}
\newacronym{qkd}{QKD}{quantum key distribution}
\newacronym{ei}{EI}{Edge Intelligence}
\newacronym{d2d}{D2D}{Device-to-device}
\newacronym{irs}{IRS}{Intelligent reflecting surfaces}
\newacronym{lis}{LIS}{Large Intelligent Surfaces}
\newacronym{noma}{NOMA}{Non-orthogonal multiple access}
\newacronym{oam}{OAM}{orbital angular momentum}
\newacronym{mec}{MEC}{mobile edge computing}
\newacronym{udhn}{UDHN}{ultra-dense heterogeneous networks}
\newacronym{rrm}{RMM}{radio resource management}
\newacronym{plmn}{PLMN}{public land mobile network}
\newacronym{thz}{THz}{Terahertz}
\newacronym{oma}{OMA}{orthogonal multiple access}
\newacronym{sic}{SIC}{successive interference cancellation}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{csi}{CSI}{channel state information}
\newacronym{cran}{CRAN}{cloud radio access network}
\newacronym{amp}{AMP}{approximate message passing}
\newacronym{hmimos}{HMIMOS}{holographic MIMO surface}
\newacronym{wpt}{WPT}{wireless power transfer}
\newacronym{ap}{APs}{access points}
\newacronym{fl}{FL}{Federated learning}
\newacronym{etsi}{ETSI}{European Telecommunications Standards Institute}

